Cooperative Design Optimization through Natural Language Interaction

Designing successful interactions requires identifying optimal design parameters. To do so, designers often conduct iterative user testing and exploratory trial-and-error. This involves balancing multiple objectives in a high-dimensional space, making the process time-consuming and cognitively demanding. System-led optimization methods, such as those based on Bayesian optimization, can determine for designers which parameters to test next. However, they offer limited opportunities for designers to intervene in the optimization process, negatively impacting the designer's experience. We propose a design optimization framework that enables natural language interactions between designers and the optimization system, facilitating cooperative design optimization. This is achieved by integrating system-led optimization methods with Large Language Models (LLMs), allowing designers to intervene in the optimization process and better understand the system's reasoning. Experimental results show that our method provides higher user agency than a system-led method and shows promising optimization performance compared to manual design. It also matches the performance of an existing cooperative method with lower cognitive load.

==> floats.tex <==
% !TEX root = ./paper.tex

\makeatletter
\@ifpackageloaded{xcolor}{}{%
  \RequirePackage{xcolor}%
}
\makeatother


\providecolor{PromptBoxBG}{named}{black}
\definecolor{PromptBoxBG}{HTML}{F2F3F5}
\definecolor{PromptBoxBorder}{HTML}{000000}

\newcommand{\PromptFigureBoxFixedContrast}[1]{
  \begingroup
  \setlength{\fboxrule}{1.0pt}
  \fcolorbox{PromptBoxBorder}{PromptBoxBG}{
    \color{black}#1
  }
  \endgroup
}


\newcommand{\figteaser}{
    \begin{teaserfigure}
        \centering
        \includegraphics[width=\textwidth]{fig/teaser.pdf}
        \caption{
            Concept of \emph{cooperative design optimization} through natural language interaction.
            The user interface designer iteratively conducts user tests to discover the best design parameters (right side).
            During this process, the designer cooperates with our system, a Bayesian optimization (BO) system extended with a large language model (LLM), to decide the condition to test next (left side).
            The cooperation is done through natural language, offering the opportunity for flexible and cognitively easy intervention in the optimization process.
        }
        \label{fig:teaser}
    \end{teaserfigure}
}

\newcommand{\figinterface}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/interface.pdf}
        \caption{
            A typical interaction scenario of cooperative design optimization with LLMs. In this scenario, a UI designer is optimizing the design of a restaurant map by providing instructions to the system (as shown at the top of the diagram). The system proposes parameters reflecting these instructions and explains the rationale behind the proposed parameters to the designer (as shown at the bottom of the diagram). The suggested parameters are automatically set on the sliders, but the designer can edit these parameter values based on the suggestions provided.
        }
        \label{fig:interface}
    \end{figure*}
}

\newcommand{\figsystemflow}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/system_flow.pdf}
        \caption{
            Overview of the system procedure.
            In each step, our system first samples $q$ candidates ($q = 8$ in this figure) using a technique called batch BO.
            Then, the LLM receives a prompt consisting of the task information, the designer's request, the previously evaluated parameter-performance pairs, and the predicted performance of the candidates.
            Finally, it chooses the parameter set that best meets the designer's request and provides its reason for that choice in natural language.
        }
        \label{fig:system_flow}
    \end{figure*}
}

\newcommand{\figappscreenshots}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/app_screenshots.pdf}
        \caption{
            Web application design tasks used in Study 1 and Study 2.
            The visual appearance of each application changes according to the associated parameter values.
            For example, in App 1 (Social Networking Service), increasing the `density of ads' parameter results in a higher number of `Buy!' icons.
            We took these screenshots with all parameters set to their medium values.
            These are based on the publicly available implementation by \citet{Mo:TIIS:24}: \url{https://github.com/georgemo535/D3MOBO}.
        }
        \label{fig:app_screenshots}
    \end{figure*}
}

\newcommand{\figuserinterface}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/user_interface.pdf}
        \caption{
        The design interface for the Cooperative: Natural Language condition used in Study 1 and Study 2. 
        (a) A set of sliders for manually adjusting parameter values, which are immediately reflected in the application.
        (b) Users can interact with the optimization system using natural language, where users can input requests to the system and receive suggested parameter values along with textual explanations.
        (c) Buttons for conducting simulated evaluations---either informal or formal---to assess the performance of the current parameter values. These buttons are used only in the user study interface to mimic user testing without involving real participants.
        (d) Objective chart showing the objective values obtained from evaluations, with the Pareto front highlighted (green line).
        (e) A parallel coordinates plot (PCP) showing the history of explored parameter values.
        }
        \label{fig:user_interface}
    \end{figure*}
}


\newcommand{\figselectingprompts}{
\begin{figure*}[t]
    \centering


    \begingroup
    \setlength{\fboxrule}{1.0pt}
    
    \PromptFigureBoxFixedContrast{%
    \begin{minipage}{\dimexpr 0.99\textwidth - 2\fboxsep - 2\fboxrule\relax}
        \sffamily
        \setlength{\parskip}{3mm}
        
        \textbf{Based on the user's request described below, select the index of the candidate point and provide a reason for your choice.}
        
        \smallskip
        
        \textbf{Task context:} \textbf{[Task Name]} \\
        \textbf{Task Description:} \textbf{[Task Description]}
        
        \smallskip
        
        \textbf{Metrics:}
        \textbf{[Metrics\_1]:}\textbf{[Explanation\_for\_Metrics\_1]}, \textbf{[Metrics\_2]:}\textbf{[Explanation\_for\_Metrics\_2]} 
        
        \medskip
        
        Hyperparameter Constraints:\\
        \textbf{[parameter\_name\_1]}\:\textbf{[parameter\_range\_1]}
        \dots
        \textbf{[parameter\_name\_n]}:\textbf{[parameter\_range\_n]}
        \\
        \textbf{[objective\_name\_1]}:\textbf{[objective\_range\_1]}
        \textbf{[objective\_name\_2]}:\textbf{[objective\_range\_2]}
        
        \medskip
        
        \textbf{User request:} \textit{\{Here is a request from designer\}}
        
        \medskip
        
        \textbf{Observed results:}
        \textbf{[configuration\_1]}\:\textbf{[performance\_1]}
        \dots
        \textbf{[configuration\_k]}\:\textbf{[performance\_k]}
        
        \medskip
        
        These candidate points are generated by a sampler for batch Bayesian optimization.
        Each candidate point includes not only the parameter names but also the following columns: \textbf{mean\_obj means \dots and variance\_obj means ... and acquisition value means ...}
        {\renewcommand{\labelitemi}{\textcolor{black}{\normalsize\raisebox{0.2ex}{\ensuremath{\bullet}}}}%
        \begin{itemize}
            \item \textbf{index: 1} \quad \textbf{[configuration\_1]} \\
            \textbf{mean\_obj1=\dots}, \textbf{variance\_obj1=\dots}, \textbf{mean\_obj2=\dots}, \textbf{variance\_obj2=\dots}, \textbf{acquisition\_value=\dots}
            \item \textbf{\dots}
            
            \item \textbf{index: $q$} \quad \textbf{[configuration\_$q$]} \\
            \textbf{mean\_obj1=\dots}, \textbf{variance\_obj1=\dots}, \textbf{mean\_obj2=\dots}, \textbf{variance\_obj2=\dots}, \textbf{acquisition\_value=\dots}
        \end{itemize}
        }
        
        \medskip
        
    \end{minipage}
    }
    \endgroup
    
    \caption{
    Prompt for candidate selection and reasoning. Bold labels with square brackets represent variables that change depending on the context. Here, $n$ refers to the number of design parameters being adjusted, and $k$ refers to the number of observed data points at that time.
    }
    \label{fig:overview_of_prompt}
\end{figure*}
}


\newcommand{\figuserstudyfirstparetofronts}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/user_study_first_pareto_fronts.pdf}
        \caption{
            Visualization of obtained Pareto fronts in Study 1.
            Green: Designer-led, Red: Cooperative, Blue: BO-led.
            Marker shapes represent individual participants.
            In general, a Pareto front located closer to the top-right of the plot indicates better design outcomes.
        }
        \label{fig:user_study_first_pareto_fronts}
    \end{figure*}
}

\newcommand{\figuserstudyfirstrelativehypervolume}{
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/user_study_first_relative_hypervolume.pdf}
        \caption{
            Boxplots of the relative hypervolume for the Designer-led, BO-led, and Cooperative conditions.
        }
        \label{fig:user_study_first_relative_hypervolume}
    \end{figure}
}

\newcommand{\figuserstudyfirstagencycomposite}{
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/user_study_first_agency_composite_score.pdf}
        \caption{
            Boxplot showing the distribution of the agency scores across conditions in Study 1. The scores are computed from three agency-related questions (see \autoref{sec:appendix_questionnaire_and_detailed_results_from_user_study_1}). Compared to the BO-led condition, both the Designer-led and the Cooperative conditions exhibit significantly higher agency.
        }
        \label{fig:user_study_first_agency_composite_score}
    \end{figure}
}

\newcommand{\firuserstudysecondparetofronts}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/user_study_second_pareto_fronts.pdf}
        \caption{
            Visualization of obtained Pareto fronts in Study 2.
            Red: Natural Language (Ours), Blue: Explicit Constraint (\citet{Mo:TIIS:24}).
            Marker shapes represent individual participants.
            In general, a Pareto front located closer to the top-right of the plot indicates better design outcomes.
        }
        \label{fig:user_study_second_pareto_fronts}
    \end{figure*}
}


\newcommand{\firuserstudysecondrelativehypervolume}{
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/user_study_second_relative_hyper_volume.pdf}
        \caption{
            Boxplots of the relative hypervolume for the Explicit Constraint (\citet{Mo:TIIS:24}) and Natural Language (Ours) conditions.
        }
        \label{fig:user_study_second_relative_hypervolume}
    \end{figure}
}


\newcommand{\firuserstudysecondnasatlxboxplot}{
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/user_study_second_nasa-tlx_overall_score.pdf}
        \caption{
        Boxplots of NASA-TLX \cite{Hart:NASATLX:1988} scores for the Explicit Constraint (\citet{Mo:TIIS:24}) and Natural Language (Ours) conditions in Study 2. The figure displays boxplots for the weighted scores calculated from responses and pairwise comparisons of all six NASA-TLX subscales.
        }
    \label{fig:user_study_second_nasa-tlx_boxplot}
    \end{figure}
}


\newcommand{\firuserstudysecondmtqboxplot}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/user_study_second_mtq_boxplot.pdf}
        \caption{Boxplots of average scores for the three Trust dimensions (Purpose, Transparency, and Utility) from the Multidimensional Trust Questionnaire \cite{Roesler:HFESAM2022} used in Study 2.
        }
    \label{fig:user_study_second_mtq_boxplot}
    \end{figure*}
}


\newcommand{\figappendixtecheval}{
    \begin{figure*}[t]
        \centering
        \includegraphics[width=\textwidth]{fig/tech_eval.pdf}
        \caption{
        Visualization of optimization results for App 1 (top), App 2 (middle), and App 3 (bottom).
            The black dots represent the five initial seed points. The red dots show the results from requests favoring Objective 1, while the blue dots show those from requests favoring Objective 2.
        }
        \label{fig:tech_eval}
        \vspace{2mm}
    \end{figure*}
}


\newcommand{\figappendixuserstudyfirstagencyboxplot}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_first_agency.pdf}
        \caption{Three agency-related questions used in Study 1 to measure participants' sense of agency during the task. Participants responded on a 7-point Likert scale, and the aggregated scores of these items form the agency composite score.}
        \label{fig:user_study_first_agency_boxplot}
    \end{figure*}
}

\newcommand{\figappendixuserstudyfirstdesignspaceunderstandingboxplot}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_first_design_space_understanding_and_exploration_experience.pdf}
        \caption{Boxplots of participants' 7-point Likert ratings on design space understanding and exploration experience for the three conditions—Designer-led, BO-led, and Cooperative—in Study 1, adapted from \cite{Mo:TIIS:24}.}
        \label{fig:user_study_first_design_space_understanding_and_exploration_experience}
    \end{figure*}
}

\newcommand{\figappendixuserstudyfirsttaskperformance}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_first_task_performance.pdf}
        \caption{These boxplots show five of the six metrics from \cite{Mo:TIIS:24} that compare the three conditions in Study 1: Designer-led, BO-led, and Cooperative. The plots illustrate (a) the total number of formal evaluations, (b) the total number of Pareto-optimal designs, (c) design space count, (d) total travel distance, and (e) mean travel distance.}
        \label{fig:appendix_user_study_first_task_performance}
    \end{figure*}
}

\newcommand{\figappendixuserstudysecondagency}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_second_agency_all.pdf}
        \caption{Boxplots of the three agency-related questions (Q1, Q2, Q3) and the agency composite score in User Study 2, based on the same items used in User Study 1. Participants responded on a 7-point Likert scale, and the composite score is calculated as ($Q1 - Q2 - Q3$).}
        \label{fig:appendix_user_study_second_agency_all}
    \end{figure*}
}


\newcommand{\figappendixuserstudysecondmtqitems}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_second_mtq_items.pdf}
        \caption{
            These boxplots show participants' 4-point Likert ratings for three subdimensions—purpose, transparency, and utility—of the Multidimensional Trust Questionnaire (MTQ) \cite{Roesler:HFESAM2022}, used to measure trust in the system. 
            Each subdimension has three items, while the performance subdimension was omitted due to the difficulty of judging goal achievement.
            In the text, we present average scores by subdimension and reverse the negatively worded utility item (``The system makes my work more difficult'') as (5 - Q1),
            ensuring that higher values consistently indicate more positive evaluations.
        }
        \label{fig:appendix_user_study_second_mtq_items}
    \end{figure*}
}

\newcommand{\figappendixuserstudyseconddesignspaceunderstandingboxplot}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_second_design_space_understanding_and_exploration_experience.pdf}
        \caption{Boxplots of participants' 7-point Likert ratings on design space understanding and exploration experience for the two Cooperative: Explicit Constraint and Cooperative: Natural Language--in Study 2, adapted from \cite{Mo:TIIS:24}.}
        \label{fig:user_study_second_design_space_understanding_and_exploration_experience}
    \end{figure*}
}

\newcommand{\figappendixuserstudysecondtaskperformance}{
    \begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{fig/appendix_user_study_second_task_performance.pdf}
        \caption{These boxplots show five of the six metrics from \cite{Mo:TIIS:24} that compare the two conditions in Study 2: Cooperative: Explicit Constraint and Cooperative: Natural Language. The plots illustrate (a) the total number of formal evaluations, (b) the total number of Pareto-optimal designs, (c) design space count, (d) total travel distance, and (e) mean travel distance.}
        \label{fig:appendix_user_study_second_task_performance}
    \end{figure*}
}
